Second-Order Actor-Critic Methods for Discounted MDPs via Policy Hessian Decomposition

We address the discounted reward setting in reinforcement learning (RL). To mitigate the value approximation challenges in policy gradient methods, actor-critic approaches have been developed and are known to converge to stationary points under suitable assumptions. However, these methods rely on first-order updates. In contrast, second-order optimization provides principled curvature-aware updates that are proven to accelerate convergence, but its application in RL is limited by the computational complexity of Hessian estimation. In this work, we analyze second-order approximations for the actor update that leverage the full curvature information of the objective as much as possible. A stable approximation requires treating the action-value function as locally constant with respect to policy parameters, which does not generally hold in policy gradient methods. We show that this approximation becomes well-justified under a two-timescale actor-critic framework, where the critic evolves on a faster timescale and can be treated as quasi-stationary during actor updates. Building on this insight, we formulate a second-order actor-critic method for the discounted reward setting that leverages Hessian-vector product (HVP) computations, resulting in a computationally efficient and stable second-order update.

==> convergenceanalysis2.tex <==
\section{Convergence Analysis}
\label{subsec:convergence}

We now analyze the convergence behavior of the proposed damped second-order
actor update. Assumptions (A1)--(A5) ensure smoothness of the objective, bounded
policy and critic derivatives, and the validity of the two-timescale
quasi-stationary critic approximation. In addition, for the convergence
argument, we require the damped curvature estimate used in the actor update to
be uniformly negative definite.

\noindent \textbf{(A6) Negative-definite damped curvature.}
Let the damped estimated Hessian $\widehat{H}_t \in \mathbb{R}^{d \times d}$ used in the actor update be calculated from $\widetilde{H}_t  \in \mathbb{R}^{d \times d}$ using a ridge-term as follows:
\[
\widehat{H}_t = \widetilde{H}_t + \lambda I .
\]
We assume that there exist constants $0<m<M<\infty$ such that
\[
-M||x||^2 \preceq x^\top\widehat{H}_tx \preceq -m||x||^2 .
\]
where $x \in \mathbb{R}^{d} $ be any arbitrary vector.
Equivalently,
\[
-\frac{||x||^2}{m} \preceq x^\top\widehat{H}_t^{-1}x \preceq -\frac{||x||^2}{M}.
\]
This assumption states that, after damping, only well-conditioned negative
definite curvature estimates are used for the actor update. But damping alone does not guarantee
negative-definiteness. So we filter out indefinite updates that persist after damping.

\paragraph{Hessian approximation error.}

Let $H_t$ denote the true curvature term and $\widehat{H}_t$ denote the practical
damped Gauss--Newton curvature estimate. The error in the curvature estimate is
bounded as
\[
\|\widehat{H}_t - H_t\|
\leq
\epsilon_H + \epsilon_{GN} + \epsilon_{\mathrm{damp}},
\]
where $\epsilon_H$ denotes the critic-induced Hessian error, $\epsilon_{GN}$
denotes the Gauss--Newton approximation error, and
$\epsilon_{\mathrm{damp}}$ denotes the bias introduced by damping. From
(A2)--(A5), the critic-tracking and two-timescale approximation imply that the
actor--critic interaction term satisfies
\[
\|\mathcal{H}_{12}^{AC}(\theta)\|
\leq
C_gC_c
\left\|
\frac{\partial \omega}{\partial \theta}
\right\|
\approx 0.
\]
Thus, the dominant practical curvature approximation error is controlled by
critic tracking, Gauss--Newton approximation, and damping.

\begin{proposition}[Convergence of the damped second-order actor update]
\label{prop:damped_second_order_convergence}
Suppose assumptions (A1)--(A6) hold. Consider the actor update
\[
\theta_{t+1}
=
\theta_t + \Delta_t,
\qquad
\Delta_t
=
-\alpha_t \widehat{H}_t^{-1}\widehat{g}_t,
\]
where $\widehat{g}_t$ is the estimated actor gradient and $\widehat{H}_t$ is the
damped positive definite curvature estimate. If the step size satisfies
\[
\alpha_t
<
\frac{2m^2M}{M(LM-m^2)}
=
\frac{2m^2}{LM-m^2},
\]
then the actor objective improves up to critic, curvature, Gauss--Newton, and
damping approximation errors. Moreover, if these approximation errors vanish
asymptotically, then
\[
\liminf_{t\to\infty}
\|\nabla J(\theta_t)\|^2
=
0.
\]
\end{proposition}
\begin{proof}
By second-order Taylor expansion with an $L$-smooth remainder, we have
\[
J(\theta_{t+1})
\geq
J(\theta_t)
+
\widehat g_t^\top \Delta_t
+
\frac{1}{2}\Delta_t^\top \widehat H_t \Delta_t
+
\frac{L}{2}\|\Delta_t\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\]
Here, the last term collects the critic-tracking, Hessian-approximation,
Gauss--Newton, and damping errors.

Using the damped second-order actor update
\[
\Delta_t
=
-\alpha_t \widehat H_t^{-1}\widehat g_t,
\]
we obtain
\begin{align}
J(\theta_{t+1})
&\geq
J(\theta_t)
-
\alpha_t
\widehat g_t^\top
\widehat H_t^{-1}
\widehat g_t
+
\frac{\alpha_t^2}{2}
\widehat g_t^\top
\widehat H_t^{-1}
\widehat H_t
\widehat H_t^{-1}
\widehat g_t
+
\frac{L\alpha_t^2}{2}
\left\|
\widehat H_t^{-1}\widehat g_t
\right\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}})
\\
&=
J(\theta_t)
-
\alpha_t
\widehat g_t^\top
\widehat H_t^{-1}
\widehat g_t
+
\frac{\alpha_t^2}{2}
\widehat g_t^\top
\widehat H_t^{-1}
\widehat g_t
+
\frac{L\alpha_t^2}{2}
\left\|
\widehat H_t^{-1}\widehat g_t
\right\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\end{align}

By Assumption (A6),
\[
-M||x||^2 \preceq x^\top\widehat{H}_tx \preceq -m||x||^2,
\qquad
-\frac{||x||^2}{m} \preceq x^\top\widehat{H}_t^{-1}x \preceq -\frac{||x||^2}{M}.
\]
Therefore,
\[
\widehat g_t^\top \widehat H_t^{-1}\widehat g_t
\leq
-\frac{1}{M}\|\widehat g_t\|^2,
\]
and
\[
\left\|
\widehat H_t^{-1}\widehat g_t
\right\|^3
\geq
-\frac{1}{m^3}\|\widehat g_t\|^3.
\]
Substituting these bounds gives
\begin{align}
J(\theta_{t+1})
&\geq
J(\theta_t)
+
\frac{\alpha_t}{M}\|\widehat g_t\|^2
-
\frac{\alpha_t^2}{2M}\|\widehat g_t\|^2
+
\frac{L\alpha_t^2}{2m^2}\|\widehat g_t\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\end{align}
Hence,
\[
J(\theta_{t+1})-J(\theta_t)
\geq
\alpha_t
\left(
\frac{1}{M}
+
\frac{\alpha_t}{2M}
-
\frac{L\alpha_t}{2m^2}
\right)
\|\widehat g_t\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\]
\noindent For monotonic improvement up to approximation error, we require
\[
\frac{1}{M}
+
\frac{\alpha_t}{2M}
-
\frac{L\alpha_t}{2m^2}
>0.
\]
Rearranging,
\[
\frac{1}{M}
>
\alpha_t
\left(
\frac{L}{2m^2}
-
\frac{1}{2M}
\right),
\]
which gives
\[
\alpha_t
<
\frac{1/M}
{\frac{L}{2m^2}-\frac{1}{2M}}
=
\frac{2m^2}{LM-m^2}.
\]
Equivalently, if \(LM \gg m^2\), this becomes the simpler sufficient condition
\[
\alpha_t
<
\frac{2m^2}{LM}.
\]

\noindent Therefore, for any step size satisfying
\[
\alpha_t
<
\frac{2m^2}{LM-m^2},
\]
there exists a constant \(G>0\) such that
\[
J(\theta_{t+1})-J(\theta_t)
\geq
G\alpha_t
\|\widehat g_t\|^2
-
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\]

\noindent Summing from \(t=0\) to \(T\), we obtain
\[
G\sum_{t=0}^{T}
\alpha_t
\|\widehat g_t\|^2
\leq
J(\theta^\star)-J(\theta_0)
+
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\]
\noindent Dividing by \(G\sum_{t=0}^{T}\alpha_t\), we get
\[
\mathbb{E}
\left[
\|\nabla J(\theta_t)\|^2
\right]
\leq
\frac{J(\theta^\star)-J(\theta_0)}
{G\sum_{t=0}^{T}\alpha_t}
+
O(\epsilon_C+\epsilon_H+\epsilon_{GN}+\epsilon_{\mathrm{damp}}).
\]
As \(T\to\infty\), if
\[
\sum_{t=0}^{T}\alpha_t \to \infty
\]
and the approximation errors vanish, then
\[
\liminf_{t\to\infty}
\|\nabla J(\theta_t)\|^2
=
0.
\]
Thus, the damped second-order actor update converges to a stationary point up to
critic, curvature, Gauss--Newton, and damping approximation errors.
\end{proof}
The above analysis shows that the proposed damped second-order actor update
converges to a neighborhood of a first-order stationary point. The size of this
neighborhood is governed by the cumulative approximation error terms arising
from critic tracking, curvature approximation, Gauss--Newton approximation, and
damping bias, i.e.,
\[
O(\epsilon_C + \epsilon_H + \epsilon_{GN} + \epsilon_{\mathrm{damp}}).
\]

Under the step-size condition
\[
\alpha_t < \frac{2m^2}{LM - m^2},
\]
and in particular the conservative sufficient bound
\[
\alpha_t < \frac{2m^2}{LM},
\]
the update guarantees monotonic improvement up to approximation error. This
yields the convergence rate
\[
\min_{0 \leq t \leq T}
\mathbb{E}\left[\|\nabla J(\theta_t)\|^2\right]
=
O\left(
\frac{1}{\sum_{t=0}^{T}\alpha_t}
\right)
+
O(\epsilon_C + \epsilon_H + \epsilon_{GN} + \epsilon_{\mathrm{damp}}).
\]

In the ideal setting where the critic tracks the optimal value function exactly
(\(\epsilon_C \to 0\)) and the curvature estimate is accurate
(\(\epsilon_H, \epsilon_{GN}, \epsilon_{\mathrm{damp}} \to 0\)), the method
recovers convergence to a true stationary point:
\[
\liminf_{t\to\infty} \|\nabla J(\theta_t)\|^2 = 0.
\]

For \textbf{ACGN2}, under log-concave policy parameterizations (e.g., softmax or
Gaussian policies), the intrinsic curvature satisfies
\[
\widetilde{H}_t \preceq 0,
\]
which implies that the damped matrix
\[
-\widetilde{H}_t + \lambda I
\]
is naturally positive definite. Consequently, ACGN2 preserves the concave
curvature structure required for stable maximization and admits a well-conditioned
second-order ascent direction. In contrast, for \textbf{ACGN1}, the inclusion of the outer-product term
introduces a positive semi-definite component that can conflict with the
intrinsic curvature, resulting in an indefinite curvature estimate. Therefore,
damping plays a critical role in ensuring that the effective update matrix
remains positive definite, thereby guaranteeing a stable ascent direction.

Overall, the analysis highlights that while both methods benefit from curvature
information, ACGN2 provides a structurally more stable approximation, whereas
ACGN1 relies more heavily on damping to control curvature-induced instability.

